GenPairX: A Hardware-Algorithm Co-Designed Accelerator for Paired-End Read Mapping

Genome sequencing has become a central focus in computational biology. A genome study typically begins with sequencing, which produces millions to billions of short DNA fragments known as reads. Read mapping aligns these reads to a reference genome. Read mapping for short reads comes in two forms: single-end and paired-end, with the latter being more prevalent due to its higher accuracy and support for advanced analysis. Read mapping remains a major performance bottleneck in genome analysis due to expensive dynamic programming. Prior efforts have attempted to mitigate this cost by employing filters to identify and potentially discard computationally expensive matches and leveraging hardware accelerators to speed up the computations. While partially effective, these approaches have limitations. In particular, existing filters are often ineffective for paired-end reads, as they evaluate each read independently and exhibit relatively low filtering ratios. In this work, we propose GenPairX, a hardware-algorithm co-designed accelerator that efficiently minimizes the computational load of paired-end read mapping while enhancing the throughput of memory-intensive operations. GenPairX introduces: (1) a novel filtering algorithm that jointly considers both reads in a pair to improve filtering effectiveness, and a lightweight alignment algorithm to replace most of the computationally expensive dynamic programming operations, and (2) two specialized hardware mechanisms to support the proposed algorithms. Our evaluations show that GenPairX delivers substantial performance improvements over state-of-the-art solutions, achieving 1575x and 1.43x higher throughput per watt compared to leading CPU-based and accelerator-based read mappers, respectively, all without compromising accuracy.

==> algorithm/cost_function.tex <==
\begin{algorithm}
\label{algo:offloader_selection}
\caption{Runtime Offloader Design}
\begin{algorithmic}[1]
    \If{operation not Flash supported}
        \State{target = DRAM}
    \Else
        \If{op1 in DRAM \& op2 in DRAM \& DRAM is idle}
            \State{target = DRAM}
        \ElsIf{Flash is idle}
            \State{target = Flash}
        \Else
            \State{target = DRAM}
        \EndIf
    \EndIf
\end{algorithmic}
\label{tab:algo}
\end{algorithm}

==> backup/background.tex <==
\section{Background}
\label{sec:background}
\rncami{We} provide an overview of \rncamii{a modern} SSD architecture and its computation resources. We describe the principles of the three NDP paradigms enabled by SSDs: in-storage processing, processing using DRAM (\pud{}), and in-flash processing. 

\subsection{SSD Overview}
Figure~\ref{fig:ssd_architecture} shows a modern NAND flash-based SSD, which consists of three main components: the SSD controller~\circled{1}, DRAM~\circled{2}, and NAND flash chips~\circled{3}. The SSD controller includes multiple general-purpose embedded cores~\circled{4} (e.g.,~\cite{arm-cortexR5,arm-cortexR8}) that execute the Flash Translation Layer (FTL) firmware~\cite{gupta2009dftl, tavakkol2018mqsim, lim2010faster, shin2009ftl, zhou2015efficient} and handle \rncami{six} key functions: 
(1) communicate with the host \rncami{using} protocols such as SATA~\cite{sata} or NVMe~\cite{nvme} over system I/O bus (e.g., PCIe\rncami{~\cite{pcie-2017}})~\circled{5}, 
(2) translate the logical address of every I/O request to a physical address, 
(3) schedule accesses to flash chips and DRAM via multiple chip and bank-level queues~\circled{6}~\circled{7} respectively.
(4) perform garbage collection~\cite{yang2014garbage, cai-procieee-2017, tavakkol2018mqsim, agrawal2008design, shahidi2016exploring, lee2013preemptible,jung2012taking, choi2018parallelizing,wu2016gcar,cai-insidessd-2018,cai-hpca-2017} to reclaim old and invalid blocks, 
(5) distribute writes (i.e., wear-leveling~\cite{cai-date-2012,cai-dsn-2015,cai-hpca-2015,cai-hpca-2017,cai-iccd-2012}) across flash blocks to uniformly wear out the SSD and improve the endurance, and  
(6) maintain FTL metadata and \rncami{cache} frequently accessed pages in \rncami{SSD's DRAM~\circled{2}}.

\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/ssd_overview.pdf}
    \caption{High-level overview of a modern SSD}
    \label{fig:ssd_architecture}
\end{figure}

A flash controller (FC)~\circled{8}\rncamii{~\cite{kim2021decoupled, kim2022networked,wu2012reducing, micheloni-insidenand-2010, microchip-16-channel-controller, cai-date-2012, cai-iccd-2012, cai-inteltechj-2013, cai-date-2013, cai-iccd-2013, cai-sigmetrics-2014, cai-hpca-2015, cai-dsn-2015, cai-hpca-2017, luo-sigmetrics-2018, cai-procieee-2017, cai-insidessd-2018, luo2018heatwatch, luo2016enabling, luo2015warm}} is a \rncami{specialized processor} that connects to flash chips\rncami{~\cite{agrawal2008design, cai-date-2012, cai-iccd-2012, cai-inteltechj-2013, cai-date-2013, cai-iccd-2013, cai-sigmetrics-2014, cai-hpca-2015, cai-dsn-2015, cai-hpca-2017, luo-sigmetrics-2018, cai-procieee-2017, cai-insidessd-2018}} via shared channels~\circled{9}. 
A modern SSD typically includes one FC per flash channel to maximize internal SSD parallelism. 
Each FC is responsible for (1) command/data transfer~\cite{micheloni-insidenand-2010,onfi-2022}, (2) data randomization~\cite{cai-procieee-2017,cai-hpca-2017,cai-insidessd-2018}, and (3) \rncami{ECC encoding/decoding}\rncamii{~\cite{cai-procieee-2017, cai-hpca-2017, cai-insidessd-2018, park2022flash,zhao2013ldpc, micheloni-insidenand-2010,tanakamaru-jssc-2013,park-asplos-2021, luo2018improving, luo2018heatwatch, luo2016enabling, luo2015warm}}. 

Each flash chip contains 1–4 independently operating dies~\circled{10}, which provide fine-grained parallelism by enabling independent access and command execution. We provide a more detailed description of the flash chip structure, and how it enables in-flash computation in \S\ref{subsec:background_ndp}.

\subsection{Near-Data Processing \label{subsec:background_ndp}}
Near-data processing (NDP)~\cite{boroumand2018google, mutlu2019enabling, mutlu.imw13,kanev.isca15, mutlu2019processing,mutlu2022modern, wang.micro2016,mckee2004reflections, mutlu.superfri15, park2022flash, hajinazar2021simdram, seshadri-micro-2017, gu-isca-2016, gao2021parabit, barbalace_blockndp_2020, augusta2015jafar, boroumand2019conda, fernandez2020natsa, singh2019napel, gao2016hrl, lee-ieeecal-2020, singh2021fpga, medal2019, liang-fpl-2019, ghiasi2022genstore, oliveira2024mimdram, nider2020processing, hsieh.isca16, ghiasi2022alp,park2024attacc,lincoln-hpca, jang2025inf, pan2024instattention, chen2022offload, jaliminchecs, kang2024isp, li2018cisc, li2023optimizing,maity2025unguided, olivier2019hexo,wei2022pimprof, weiner2022tmo, yang2023lambda, chen2024aresflash, kabra2025ciphermatch, kim2025crossbit,kang-tc-2021, chen2024search, wong2024tcam, besta2021sisa, seshadri-arxiv-2019, li-micro-2017, seshadri-micro-2013, seshadri-arxiv-2016-pum, deng-dac-2018,xin-hpca-2020, gao-micro-2019, seshadri-ieeecal-2015, yuksel2024functionally, yuksel2025dram, yuksel2024simultaneous, park2016storage, mailthody-micro-2019, kim-fast-2021, kang-msst-2013, torabzadehkashi-pdp-2019, seshadri-osdi-2014, wang-eurosys-2019,acharya-asplos-1998,keeton-sigmod-1998, wang2016ssd, koo-micro-2017, tiwari-fast-2013, tiwari-hotpower-2012, boboila-msst-2012, bae-cikm-2013,torabzadehkashi-ipdpsw-2018, pei-tos-2019, do-sigmod-2013, kim-infosci-2016, riedel-computer-2001,riedel-vldb-1998, liang-atc-2019,cho-wondp-2013, jun2015bluedbm, ajdari-hpca-2019, jun-hpec-2016, kim-sigops-2020, lee2022smartsage, li2023ecssd, ruan2019insider, wang2016ssd1, li-atc-2021, jeong-tpds-2019, mao2012cache, gouk2024dockerssd, ghiasi_megis_2024, kang-micro-2021, yavits2021giraf, kim2023optimstore, lim-icce-2021, narasimhamurthy2019sage, jun-isca-2018, fakhry2023review, jo2016yoursql, chen2025reis, mahapatra2025rag, torabzadehkashi2019catalina, torabzadehkashi2018compstor, olgun2023dram, gao2022fracdram,wong2025anvil, perach-arxiv-2022, gokhale1995processing, patterson-ieeemicro-1997, oskin1998active, kang1999flexram} mitigates the data movement bottleneck by enabling computation closer to the data, typically \rncami{inside} or near memory or storage \rncami{arrays}. 
SSDs are well-suited for NDP because they inherently include three heterogeneous computation resources: (1) SSD controller cores, which support general-purpose computation \rncami{capability}, (2) \rncamii{SSD-internal} DRAM, which enables fast, parallel bulk bitwise and arithmetic operations, and (3) NAND flash chips, which \rncami{enable parallel} in-place bulk bitwise and arithmetic operations. 

\head{In-Storage Processing (\isp{})}
The SSD controller cores\rncami{~\cite{arm-cortexR5,arm-cortexR8,marvellsc5bravera, armssdcontroller, cai-procieee-2017, micheloni2013inside, cheong2018flash, hatanaka2012nand, liao2012multi, park2006high, do2019improving, dirik2009performance, takeuchi2009novel,kim2021decoupled, kim2022networked}} typically execute FTL firmware and handle host communication, but they can be repurposed to perform general-purpose computations. 
Prior works (e.g.,~\cite{park2016storage, kabra2025ciphermatch, mailthody-micro-2019, kim-fast-2021, kang-msst-2013, torabzadehkashi-pdp-2019, wang-eurosys-2019,acharya-asplos-1998,keeton-sigmod-1998, tiwari-fast-2013, tiwari-hotpower-2012, boboila-msst-2012, bae-cikm-2013,torabzadehkashi-ipdpsw-2018, pei-tos-2019, do-sigmod-2013, kim-infosci-2016, riedel-computer-2001,riedel-vldb-1998, liang-atc-2019,cho-wondp-2013, jun2015bluedbm, lee-ieeecal-2020, ajdari-hpca-2019,liang-fpl-2019,jun-hpec-2016, kang-tc-2021, kim-sigops-2020, lee2022smartsage, li2023ecssd, ruan2019insider, wang2016ssd1, li-atc-2021, jeong-tpds-2019, mao2012cache, gouk2024dockerssd, ghiasi_megis_2024, ghiasi2022genstore, kang-micro-2021, yavits2021giraf, kim2023optimstore, lim-icce-2021, narasimhamurthy2019sage, jun-isca-2018, fakhry2023review, gu-isca-2016, yang2023lambda, jo2016yoursql, chen2025reis, wang2016ssd, seshadri-osdi-2014, mahapatra2025rag, pan2024instattention, torabzadehkashi2019catalina, lee2017extrav, wang2024beacongnn, yu2024cambricon, pan2024instinfer}) demonstrate that these embedded cores can accelerate \rncami{various} tasks \rncami{including filtering, aggregation, encryption, compression and search}. 
% While NDP using SSD controller cores reduces host-SSD data movement, their limited SIMD parallelism (e.g., 32-bit registers in ARM Cortex-R5~\cite{arm-cortexR5}) constrains performance for data-parallel workloads.
\rncami{\rncamii{Limited} SIMD parallelism (e.g., 32-bit registers in ARM Cortex-R5~\cite{arm-cortexR5}) in the SSD controller cores reduces the computation throughput, making \isp{} less effective for data-parallel workloads.}

\head{Processing-using-DRAM in SSD (\pud{})} 
Modern SSDs integrate a \rncami{set of} low-power DRAM \rncami{chips} (e.g., 4GB LPDDR4 for 4TB SSDs~\cite{samsung-980pro}) to store metadata and cache frequently accessed pages\rncami{~\cite{gupta2009dftl, tavakkol2018mqsim, lim2010faster, shin2009ftl, zhou2015efficient, cai-procieee-2017, lim_faster_2010,sun_leaftl_2023, wang_learnedftl_nodate, ma_lazyftl_2011, zhou_efficient_2015}}.
This DRAM subsystem exposes high internal bandwidth and parallelism, making it a well-suited substrate for NDP.
Figure~\ref{fig:processing_using_ssd_dram} shows DRAM organization and the architectural principles that enable \pud{}. 
Each DRAM module consists of 8–16 chips, and each chip contains several independent DRAM banks~\circleds{2a} capable of serving requests in parallel.
A bank is composed of multiple mats (subarrays\rncami{~\cite{salp,seshadri-micro-2013, lee.hpca13, seshadri-micro-2017, chang-hpca-2016, chang.hpca14, lee.hpca15, seshadri_fast_2015, chargecache, lee.sigmetrics17}})~\circleds{2b}, each composed of cell arrays~\circleds{2c} organized as rows and columns. 
The mat selector\rncami{~\cite{oliveira2024mimdram}}~\circleds{2d} connects a chosen mat to global bitlines and shared sense amplifiers, while local row decoders~\circleds{2e} activate local wordlines~\circled{2f} to access stored bits. 
The activated row is latched in a row buffer~\circleds{2g}. The global wordlines~\circleds{2h} coordinate access across mats. Each DRAM cell~\circled{2i} stores a single bit using a capacitor-transistor pair. 
% This hierarchical structure is key to enabling \pud{}, because activating multiple rows or coordinating operations across mats allows DRAM to perform bulk bitwise and arithmetic operations in situ. 

\begin{figure}[b]
    \centering    
    \includegraphics[width=\linewidth]{images/dram_background.pdf}
    \caption{Overview of processing-using-DRAM}
    \label{fig:processing_using_ssd_dram}
\end{figure}

\rncami{Processing using DRAM (PuD) techniques \rncamii{leverage} DRAM's intrinsic operational principles to perform computation directly within memory arrays. 
Prior works \rncamii{(e.g.,~\cite{seshadri-micro-2017, hajinazar2021simdram, oliveira2024mimdram, besta2021sisa, seshadri-arxiv-2019, li-micro-2017, seshadri-micro-2013, seshadri-arxiv-2016-pum, deng-dac-2018, xin-hpca-2020, gao-micro-2019, seshadri-ieeecal-2015, yuksel2024functionally, yuksel2025dram, yuksel2024simultaneous, mutlu2025memory, mutlu2024memory, lenjani_fulcrum_2020, silentpim, park2024attacc, leitersdorf2023aritpim, olgun2022pidram, olgun2023dram, peng_chopper_2023, gao2022fracdram, roy-2021-jetcas})} show that careful orchestration of ACT (row activation) and PRE (precharge) commands enables a range of primitive operations (e.g., AND, OR, NOT, MAJORITY) in a highly parallel manner within the DRAM chips. 
RowClone~\cite{seshadri-micro-2013} demonstrates that consecutively activating two rows within the same DRAM subarray enables fast bulk data copy and initialization by transferring data through shared sense amplifiers. 
Ambit~\cite{seshadri-micro-2017} exploits triple-row activation to compute the bitwise MAJORITY (AND and OR by extension) function, and implements bitwise NOT using sense amplifiers, with DRAM circuit modifications.  

Building on these techniques, SIMDRAM~\cite{hajinazar2021simdram} introduces a software-hardware co-designed framework that maps arbitrary logic circuits composed of AND, OR, and NOT gates onto the Ambit substrate. SIMDRAM enables complex operations (e.g., multiplication, addition, convolution) to be \rncamii{performed} entirely within the DRAM chips. 
MIMDRAM~\cite{oliveira2024mimdram} improves programmability and applicability of the Ambit substrate by (1) supporting finer-granularity operations than full-row execution, and (2) providing compiler support that transparently transforms applications to exploit bulk-bitwise execution.
\rncamii{Recent studies on commercial-off-the-shelf (COTS) DRAM chips demonstrate that existing DRAM chips\rncamiii{~\cite{mutlu2025memory, mutlu2024memory, yuksel2025dram, yuksel2025columndisturb, yuksel2025pudhammer, yuksel2024simultaneous, yuksel2024functionally, olgun2023dram, gao-micro-2019, gao2022fracdram, olgun2021quactrng, kim-hpca-2019 }} are capable of performing all of these operations by violating specific timing parameters in the memory controllers, without modifying the DRAM chip and the DRAM interface.}

Compared to execution on SSD controller cores, \pud{} \rncamii{enables} executing computations in DRAM chips enables massive internal parallelism, and significantly improves performance and energy efficiency. However, \pud{} operates on data in the DRAM, which requires transferring operands from flash chips via bandwidth-limited flash channels. These data transfers introduce additional latency and flash channel contention. 
% Hence, \pud{}'s effectiveness depends on the operand locality, data reuse, and data movement from flash chips to DRAM.
}

% Prior works (e.g.,~\cite{seshadri-micro-2017, hajinazar2021simdram, oliveira2024mimdram, besta2021sisa, seshadri2020indram, li-micro-2017, seshadri-micro-2013, seshadri-arxiv-2016-pum, deng-dac-2018,xin2020elp2im, gao2020computedram, seshadri-ieeecal-2015, yuksel2024functionally, yuksel2025dram, yuksel2025columndisturb, yuksel2025pudhammer, yuksel2024simultaneous, oliveira2024mimdram}) show that careful orchestration of ACT (row activation) and PRE (precharge) commands enables operations such as AND, OR, NOT, MAJORITY, addition, and predication in a highly parallel manner within the DRAM.
% As a result, \pud{} achieves significant performance improvement over execution using SSD controller cores. However, it requires that operands reside in DRAM, which necessitates transferring data from flash chips via bandwidth-limited flash channels. These data transfers introduce additional latency and contention. Hence, \pud{}'s effectiveness depends on the locality of the operands and the cost of fetching data into DRAM. 

\head{In-Flash Processing (IFP)}
Figure~\ref{fig:in_flash_processing} shows the organization of a NAND flash chip and the principles that enable computations inside the flash array. 
A NAND flash chip~\circleds{3a}\rncamii{~\cite{stoica2019understanding, grupp2009characterizing, cai-procieee-2017, yucai-thesis, nadig2023venice, dirik2009performance, micheloni2013inside, cai.bookchapter18.arxiv, cai-insidessd-2018, cai-hpca-2017, cai-date-2012, cai-dsn-2015, cai-iccd-2012, cai-date-2013, cai-hpca-2015, cai-iccd-2013, cai-inteltechj-2013, cai-sigmetrics-2014}} contains 1-4 independent dies~\circleds{3b}, each capable of operating concurrently.
\rncami{Each flash die has multiple planes~\circleds{3c} (typically 1 to 4) that share the flash die's peripheral circuitry for row decoding, sensing, and programming. Each plane holds thousands of blocks~\circleds{3d}.}
Each block consists of hundreds of pages. Each page corresponds to a row of flash cells connected to a single wordline in a block. Read/write operations are performed at page granularity (e.g., 16KB). 
Planes within the same die operate concurrently (\rncami{enabling} multi-plane operations), but only when accessing pages at the same offset. 
Vertically stacked flash cells (typically \rncami{consisting of 24-1024 cells}) connected in series form NAND strings~\circleds{3e} that connect to bitlines (BLs). Multiple NAND strings across different BLs constitute a sub-block~\circled{3f}. 
\rncami{A flash cell}~\circleds{3g} \rncami{stores} bits \rncami{in terms of its} threshold voltage: \rncami{a cell in the programmed state (0) has a high threshold voltage, whereas an erased cell (1) has a low threshold voltage. During reads, a programmed cell behaves as an open switch, and an erased cell operates as a resistor.}

\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{images/nand_background.pdf}
\caption{Overview of in-flash processing}
\label{fig:in_flash_processing}
\end{figure}

IFP techniques\rncami{~\cite{park2022flash, gao2021parabit, chen2024aresflash, kabra2025ciphermatch, kim2025crossbit, kang-tc-2021, chen2024search, wong2024tcam}} exploit the flash chip's structure to perform bulk bitwise and arithmetic operations within the flash chips. 
Flash-Cosmos~\cite{park2022flash} enables bitwise AND~\circleds{3h} (OR~\circled{3i}) by simultaneously activating multiple wordlines within (across) blocks.
Several works~\cite{chen2024aresflash,kabra2025ciphermatch,gao2021parabit} control the latches (S-latch, D-latch)~\circleds{3j} in the page buffer within the flash die's peripheral circuitry to enable more complex operations such as addition and multiplication~\circleds{3k}.
These techniques exploit both bit-level and array-level parallelism within the SSD to enable efficient in-place computation. 
While \ifp{} eliminates data movement overhead and enables high parallelism, it supports a limited set of operations and is \rncami{therefore} less suitable for workloads that require complex computations.

==> backup/introduction.tex <==
\section{Introduction \label{sec:introduction}}
Near-data processing (NDP) techniques \rncamii{(e.g., \cite{boroumand2018google, mutlu2019enabling, mutlu.imw13,kanev.isca15, mutlu2019processing,mutlu2022modern, wang.micro2016,mckee2004reflections, mutlu.superfri15, park2022flash, hajinazar2021simdram, seshadri-micro-2017, gu-isca-2016, gao2021parabit, barbalace_blockndp_2020, augusta2015jafar, boroumand2019conda, fernandez2020natsa, singh2019napel, gao2016hrl, lee-ieeecal-2020, singh2021fpga, medal2019, liang-fpl-2019, ghiasi2022genstore, oliveira2024mimdram, nider2020processing, hsieh.isca16, ghiasi2022alp,park2024attacc,chen2022offload,li2018cisc, li2023optimizing,maity2025unguided, olivier2019hexo,wei2022pimprof, weiner2022tmo, yang2023lambda, lincoln-hpca, jang2025inf, pan2024instattention, jaliminchecs, kang2024isp})} alleviate the performance and energy overheads caused by \emph{data movement} in modern computing systems by enabling computation close to where data resides\rncami{~\cite{mutlu2022modern, mutlu2025memory, mutlu2019processing}}. 
In \rncami{processor-centric} computing systems, the performance and energy efficiency of modern data-intensive applications 
\rncamii{(e.g., databases~\cite{doty1980magnetic, elmasri2007fundamentals, kocberber2013meet, augusta2015jafar, Oracle, idreos2012monetdb, wu2014q100, chan1998bitmap, oneil-ideas-2007, li-vldb-2014, li-sigmod-2013, goodwin-SIGIR-2017, seshadri-micro-2013, seshadri-micro-2017, seshadri-ieeecal-2015, hajinazar2021simdram, fastbit, wu-icde-1998, guz-ndp-2014, redis-bitmaps, kabra2025ciphermatch}, 
web search~\cite{ccetin2016blind, pugsley2014ndc, cho-wondp-2013, janapa2010web, ayers2018memory, zhu2013high, reddi2011mobile}, 
data analytics~\cite{jia2017understanding, jun2015bluedbm, perach-arxiv-2022, seshadri-micro-2017, torabzadehkashi-pdp-2019, lee-ieeecal-2020, jun-isca-2018, choi2015energy, panda2014data, jun2014scalable, wang2017xpro, tiwari-fast-2013, boboila-msst-2012, gao.pact15}, 
genomics~\cite{alser-bioinformatics-2017, loving-bioinformatics-2014, xin-bioinformatics-2015, cali-micro-2020, kim-genomics-2018, lander-nature-2001, altschul-jmb-1990, myers-jacm-1999, ghiasi_megis_2024, ghiasi2022genstore, papageorgiou2018genomic, cali-micro-2020, soysal2025mars, alkan.naturegenetics09}, 
graph processing~\cite{shim2022gp3d, zhang2018graphp, ahn2015scalable, zhuo2019graphq, huang2020heterogeneous, song2018graphr, dai2018graphh, beamer-SC-2012, besta2021sisa, li-dac-2016, gao2021parabit, hajinazar2021simdram}, 
\rncamii{machine learning~\cite{ankit2019puma, low.vldb12, wang2020survey, sheng2023flexgen,pan2024instattention,jang2025inf, boroumand2021google, he2025papi, gu2025pim, park2024attacc, lincoln-hpca, lee2025aif, kim2023optimstore, LSTM, reinforce1992, gomezluna2022isvlsi, qlearning_ML_1992, wang2024beacongnn, yu2024cambricon, pan2024instinfer}}, 
cryptography~\cite{tuyls-springer-2005, manavski-spcom-2007, nejatollahi2020cryptopim, han-spie-1999, lee2005architecture, hajiabadi2025cassandra, lemay2021cryptographic, devadas2022designing, wang2022eager, diffie2022new, chang2011workload}, mobile workloads~\cite{boroumand2018google, wang2013architectural, liang2025ariadne, olivier2019hexo, halpern2016mobile, gupta2024relief, mobile-tensorflow, reddi2011mobile})}
are limited by the data movement between the compute units (e.g., CPU, GPU) and the memory \rncami{system}.
\rncami{Many} of these workloads (e.g., graph processing, sorting, sparse matrices) perform simple computations (e.g., bitwise operations, \rncami{comparisons}) with low arithmetic intensity, making data movement the dominant cost during execution.
NDP reduces unnecessary \rncami{data movement} and enables efficient use of memory and storage bandwidth\rncami{~\cite{mutlu2025memory, mutlu2022modern, mutlu2019processing, mutlu2019enabling, mutlu2024memory,ghose2019processing}}.

A solid-state drive (SSD) (e.g.,~\cite{seagate,samsung-980pro, adatasu630,intelqlc,intels4510, intelp4610, nadig2023venice, cai-procieee-2017, micheloni-insidenand-2010, micheloni2013inside, inteloptane, SSD_fast, SSD_slow, LSSD}) is well-suited for NDP \rncami{due to at least} three reasons.
First, it stores large application datasets that often exceed main memory capacity. 
Second, it enables three heterogeneous NDP paradigms: \rncami{1)} processing using general-purpose embedded cores in the SSD controller (in-storage processing (\isp{}))~\cite{park2016storage, kabra2025ciphermatch, mailthody-micro-2019, kim-fast-2021, kang-msst-2013, torabzadehkashi-pdp-2019, seshadri-osdi-2014, wang-eurosys-2019,acharya-asplos-1998, keeton-sigmod-1998, koo-micro-2017, tiwari-fast-2013, tiwari-hotpower-2012, boboila-msst-2012, bae-cikm-2013,torabzadehkashi-ipdpsw-2018, pei-tos-2019, do-sigmod-2013, kim-infosci-2016, riedel-computer-2001,riedel-vldb-1998, liang-atc-2019,cho-wondp-2013, jun2015bluedbm, lee-ieeecal-2020, ajdari-hpca-2019,liang-fpl-2019,jun-hpec-2016, kang-tc-2021, kim-sigops-2020, lee2022smartsage, li2023ecssd, ruan2019insider, wang2016ssd1, jeong-tpds-2019, mao2012cache, gouk2024dockerssd, ghiasi_megis_2024, ghiasi2022genstore, kang-micro-2021, yavits2021giraf, kim2023optimstore, lim-icce-2021, narasimhamurthy2019sage, jun-isca-2018,  fakhry2023review, gu-isca-2016, yang2023lambda, jo2016yoursql, chen2025reis, li-atc-2021, wang2016ssd, mahapatra2025rag, pan2024instattention, torabzadehkashi2019catalina, wang2024beacongnn, yu2024cambricon, pan2024instinfer}, 
\rncami{2)} processing using DRAM in the SSD (\pud{})\rncami{~\cite{seshadri-micro-2017, hajinazar2021simdram, oliveira2024mimdram, besta2021sisa,seshadri-arxiv-2019, li-micro-2017, seshadri-micro-2013, seshadri-arxiv-2016-pum, deng-dac-2018,xin-hpca-2020, gao-micro-2019, yuksel2025dram, olgun2023dram,gao2022fracdram, yuksel2024functionally, seshadri-ieeecal-2015, yuksel2024simultaneous}}, and 
\rncami{3)} in-flash processing (\ifp{})\rncami{~\cite{park2022flash, gao2021parabit, chen2024aresflash, kim2025crossbit,wong2024tcam, wong2025anvil, chen2024search, choi2020flash, chun2022pif, lee2025aif, wang2018three,  kabra2025ciphermatch, kang-tc-2021}} (see \S\ref{sec:background} for details). These in-situ computation capabilities reduce unnecessary data movement between the host \rncami{processor} and the SSD, and ease the burden on the memory hierarchy.
Third, \rncami{an SSD} provides high internal parallelism for concurrent data access and computation.

While a large \rncami{number} of prior works (e.g., \cite{park2016storage, kabra2025ciphermatch, mailthody-micro-2019, kim-fast-2021, kang-msst-2013, torabzadehkashi-pdp-2019, seshadri-osdi-2014, wang-eurosys-2019,acharya-asplos-1998,keeton-sigmod-1998, wang2016ssd, koo-micro-2017, tiwari-fast-2013, tiwari-hotpower-2012, boboila-msst-2012, bae-cikm-2013,torabzadehkashi-ipdpsw-2018, pei-tos-2019, do-sigmod-2013, kim-infosci-2016, riedel-computer-2001,riedel-vldb-1998, liang-atc-2019,cho-wondp-2013, jun2015bluedbm, lee-ieeecal-2020, ajdari-hpca-2019,liang-fpl-2019,jun-hpec-2016, kang-tc-2021, kim-sigops-2020, lee2022smartsage, li2023ecssd, ruan2019insider, wang2016ssd1, li-atc-2021, jeong-tpds-2019, mao2012cache, gouk2024dockerssd, ghiasi_megis_2024, ghiasi2022genstore, kang-micro-2021, yavits2021giraf, kim2023optimstore, lim-icce-2021, narasimhamurthy2019sage, jun-isca-2018, fakhry2023review, gu-isca-2016, yang2023lambda, jo2016yoursql, chen2025reis, park2022flash, gao2021parabit, chen2024aresflash, soysal2025mars, lee2017extrav}) \rncami{propose} SSD-based NDP techniques, they have two key limitations.
First, these techniques operate largely in isolation, offloading parts of the application to \emph{only} one or two SSD computation resources, which prevents them from exploiting the SSD's full computational potential.
For example, Active Flash~\cite{tiwari-fast-2013} offloads data analytics kernels to SSD controller cores (ISP) and
Flash-Cosmos~\cite{park2022flash} exploits only flash chips to accelerate bulk bitwise operations via in-flash processing.  
Second, these techniques are typically application-specific and \rncami{\emph{not}} programmer-transparent, which \rncami{limits their general applicability}. For example, MARS~\cite{soysal2025mars} accelerates raw signal genome analysis in the SSD by adding specialized hardware units in the SSD DRAM and the SSD controller, but it relies on custom data layouts and the explicit identification of offloadable sections by the programmer.
\rncami{The need for such programmer} intervention limits the generality of these techniques and their \rncami{ease of} adoption in modern storage \rncamii{and system} stacks.

\noindent \head{Limitations of Prior Offloading Approaches} 
To our knowledge, \emph{no} prior work exploits \rncamii{\emph{multiple}} SSD computation resources in a \rncamii{\emph{general-purpose}} and \rncamii{\emph{application-transparent}} manner. 
\rncami{Several} prior NDP offloading techniques (e.g.,\ak{\cite{ghiasi2022alp,park2024attacc, chen2022offload, hsieh.isca16, li2018cisc, li2023optimizing, maity2025unguided, olivier2019hexo, wei2022pimprof, weiner2022tmo, wolski2008using, yang2023lambda, hadidi2017cairo, wu2020tuning, alsop2024pim, kim2017toward, jiang20243}}) propose partitioning and mapping applications for execution between \rncami{specifically} the host and NDP units near main memory (e.g., 3D stacked memory with \rncami{general-purpose} cores in its logic layer).
\rncami{Unfortunately,} adapting these techniques to SSD-based NDP provides limited benefits because they (1) do \rncami{\emph{not}} account for the architectural heterogeneity of the SSD computation resources, which vary in their parallelism, access granularities, and computation capabilities, and (2) optimize for \emph{only} a limited set of system-level metrics such as bandwidth utilization (e.g.,~\cite{hsieh.isca16}) or data movement cost (e.g.,~\cite{ghiasi2022alp}), while ignoring key factors such as computation resource utilization\rncami{, \rncamii{operand location,} and data dependencies}.

We study the effectiveness of two prior offloading models, \bw{} \rncami{(e.g.,~\cite{wolski2008using, yang2023lambda, hsieh.isca16, hadidi2017cairo, wu2020tuning, alsop2024pim})} and \dm{} \rncami{(e.g.,~\cite{ghiasi2022alp, kim2017toward, wei2022pimprof,jiang20243})}, when applied to offloading computations within an SSD. 
Our motivational study shows that the best-performing prior model, \dm{}, shows an average performance gap of 2.5$\times$ compared to an \ideal{} offloading approach that assumes no resource contention and always selects \rncamii{the} resource with the lowest computation latency (see \S\ref{subsec:motivation_effectiveness} for more \rncami{detail}). 
These results show the need for an offloading mechanism that fully exploits the heterogeneity of SSD computation resources and makes workload- and system-aware offloading decisions. 

% \textbf{Our goal} is to fundamentally alleviate the data-movement bottleneck by coordinating computations across multiple SSD computation resources and making offloading decisions that are both workload- and system-aware.
\rncami{\textbf{Our goal} is to enable programmer-transparent near-data processing in SSDs that (1) \rncamii{schedules and} coordinates computation across \rncamii{multiple} heterogeneous SSD computation resources and (2) makes offloading decisions that are aware of both workload characteristics and dynamic system conditions, and (3) improves the performance and energy efficiency of a wide range of applications.
To this end, we propose \textit{\textbf{\namePaper{}}}, a general-purpose programmer-transparent NDP framework that dynamically offloads fine-grained computations (at instruction granularity) to SSD controller cores, SSD DRAM chips, and flash chips.}

\namePaper{} consists of two key steps. 
First, \namePaper{} performs compile-time vectorization to identify offloadable code regions (e.g., loops with computations) and transforms them into SIMD operations that match the internal bit-level parallelism of an SSD.
Second, at runtime, \namePaper{} (i) determines the most suitable SSD computation resource to execute each vector operation using a holistic cost function, which is based on six key factors: operation type, operand location, data dependencies, resource utilization, data movement costs\rncami{,} and computation latencies, (ii) translates each vector operation to the native instruction set architecture (ISA) of the chosen SSD computation resource, and (iii) dispatches the transformed instruction to the chosen resource's execution queue. 

We evaluate \namePaper{} and six prior NDP
techniques\rncami{~\cite{arm-cortexR8, oliveira2024mimdram, park2022flash, chen2024aresflash, yang2023lambda, ghiasi2022alp}} using an event-driven SSD simulator.\footnote{We develop \namePaper{}'s simulator due to the lack of SSD simulators that support NDP. Our \rncami{simulator} inherits its core SSD model from the state-of-the-art SSD simulator, MQSim~\cite{tavakkol2018mqsim, mqsim-github}. Our NDP extensions (i.e., models for SSD computation resources) are calibrated using real-device characterization studies (e.g.,~\cite{park2022flash, chen2024aresflash}) and open-source \rncamii{infrastructures} (e.g.,~\cite{luo2023ramulator2, oliveira2024mimdram, qemu}) from prior works (See \S\ref{subsec:methodology_modeling}).} 
Our evaluation includes six data-intensive real-world applications (see \S\ref{sec:methodology}) that cover diverse \rncami{computation} and access patterns.
\namePaper{} outperforms the best-performing prior offloading policy\rncami{~\cite{ghiasi2022alp}} by 1.8$\times$ and reduces energy consumption by 46\% on average.
% demonstrating the benefits of coordinated, fine-grained offloading across heterogeneous SSD computation resources. 

This work makes the following key contributions:
\begin{itemize}[leftmargin=*]
\item We demonstrate that prior NDP offloading approaches offer limited benefits when adapted to SSDs because they (1) do not account for the architectural heterogeneity of SSDs, and (2) optimize for only a limited set of system-level metrics (e.g., data movement or bandwidth). 
\item We propose \namePaper{}, the first general-purpose programmer-transparent NDP framework that enables fine-grained \rncamii{(i.e., instruction-granularity)} offloading across \rncami{multiple} heterogeneous SSD computation resources. 
\namePaper{} dynamically determines the most suitable computation resource for each instruction using a holistic cost function that is based on multiple application and system characteristics.
\item We evaluate \namePaper{} and \rncami{six} prior offloading techniques on six real-world data-intensive applications. \namePaper{} provides significant performance and energy benefits over prior offloading techniques across all workloads.
\end{itemize}

==> backup/motivation.tex <==
\section{Motivation}
\rncamiii{We demonstrate} the need for an effective offloading policy for SSD-based NDP. We (1) describe the limitations of NDP techniques proposed for SSDs, (2) present a case study that demonstrates the need for offloading computations across \rncamiii{multiple} SSD computation resources, and (3) quantitatively demonstrate that prior offloading techniques proposed for other NDP architectures fall short when adapted to SSDs.

A modern SSD contains multiple heterogeneous computation resources, including general-purpose embedded controller cores, SSD-internal DRAM, and NAND flash chips (see \S\ref{subsec:background_ndp}). Each computation resource enables an NDP paradigm with different strengths and limitations. We describe the strengths and limitations of each of these computation paradigms in \S\ref{subsec:background_ndp}.

\head{Limitations of SSD-based NDP Techniques}
A large body of prior work (e.g., \cite{park2016storage,   kabra2025ciphermatch, mailthody-micro-2019, kim-fast-2021, kang-msst-2013, torabzadehkashi-pdp-2019, seshadri-osdi-2014, wang-eurosys-2019,acharya-asplos-1998,keeton-sigmod-1998, wang2016ssd, koo-micro-2017, tiwari-fast-2013, tiwari-hotpower-2012, boboila-msst-2012, bae-cikm-2013,torabzadehkashi-ipdpsw-2018, pei-tos-2019, do-sigmod-2013, kim-infosci-2016, riedel-computer-2001,riedel-vldb-1998, liang-atc-2019,cho-wondp-2013, jun2015bluedbm, lee-ieeecal-2020, ajdari-hpca-2019,liang-fpl-2019,jun-hpec-2016, kang-tc-2021, kim-sigops-2020, lee2022smartsage, li2023ecssd, ruan2019insider, wang2016ssd1, li-atc-2021, jeong-tpds-2019, mao2012cache, gouk2024dockerssd, ghiasi_megis_2024, ghiasi2022genstore, kang-micro-2021, yavits2021giraf, kim2023optimstore, lim-icce-2021, narasimhamurthy2019sage, jun-isca-2018, fakhry2023review, gu-isca-2016, yang2023lambda, jo2016yoursql, chen2025reis, park2022flash, gao2021parabit, chen2024aresflash, soysal2025mars, lee2017extrav, kim2025crossbit, chen2024search, wong2024tcam, pan2024instattention, choi2015energy}) proposes SSD-based NDP techniques. These techniques have two key limitations.

First, these techniques operate largely in isolation and map specific portions of an application to \emph{only} one or two SSD computation resources, which prevents them from exploiting the SSD's full computational potential.
For instance, Active Flash~\cite{tiwari-fast-2013} offloads data analytics kernels to SSD controller cores (ISP), and Flash-Cosmos~\cite{park2022flash} accelerates bulk bitwise operations directly within NAND flash chips (IFP).
Our motivational experiments in \S\ref{subsec:motivation_effectiveness} on six real-world workloads show that ISP and IFP, in isolation, underperform by 1.8$\times$ and 1.9$\times$ on average compared to an offloading approach~\cite{ghiasi2022alp} that leverages \rncamiii{\emph{multiple}} SSD computation resources.  

Second, these techniques are typically application-specific and \emph{not} programmer-transparent. 
For example, MARS~\cite{soysal2025mars} accelerates raw signal genome analysis\rncamiii{~\cite{firtina2023rawhash, firtina2024rawhash2, firtina2024rawsamble, lindegger2024rawalign, eris2025rawbench}} by performing computations within the SSD-internal DRAM and the SSD controller. MARS requires the programmer to explicitly identify offloadable sections and manage data placement \rncamiii{and code scheduling} to enable in-situ computations. The need for such programmer intervention limits \rncamiii{generality} and their ease of adoption in modern storage and system stacks. 

\subsection{Case Study on Offloading Computations in SSD \label{subsec:motivation_casestudy}}
Offloading computation across multiple SSD computation resources is key to exploiting the SSD's full computational potential. To study how different workloads interact with SSD computation resources, we conduct a case study that examines performance bottlenecks (i.e., data movement or computation) across three execution models (see \S\ref{sec:methodology} for our experimental methodology):
(1) Outside-storage processing (OSP) on host CPU or GPU, 
(2) In-storage processing (\isp{}) on SSD controller cores, and 
(3) In-flash processing (\ifp{}) within flash chips. 
We exclude \pud{} from this study because \pud{} has similar data movement overheads as \isp{}, but provides higher computation parallelism. 
\fig~\ref{fig:motivation_casestudy} presents our analyses for three categories of workloads, I/O-intensive, more compute-intensive, and mixed workloads.

\begin{figure}[b]
\centering
\includegraphics[width=\linewidth]{images/motivation_casestudy.pdf}
\caption{Case Study on offloading computations across
computation resources.}
\label{fig:motivation_casestudy}
\end{figure}

\head{I/O-Intensive Workloads} For workloads (e.g., databases~\cite{Oracle, li-sigmod-2013}, bitmap indices~\cite{fastbit, redis-bitmaps, chan1998bitmap, seshadri-ieeecal-2015}) dominated by data transfer, OSP is limited by the host-SSD data movement. 
\isp{} outperforms OSP by 30\% by reducing host-SSD data movement, but \isp{}'s performance is limited by the significant data movement between the flash chips and the SSD controller via bandwidth-limited flash channels. 
\rncamiii{IFP outperforms OSP by 70\% by executing computations directly within the flash chips and largely reducing the data movement}. 
Naively combining IFP and ISP reduces performance by 15\% compared to IFP, because the additional data movement overhead between flash chips and the controller offsets the benefits of IFP’s \rncamiii{highly} parallel computation capability.

\head{More Compute-Intensive Workloads} 
For more compute-intensive workloads (e.g., encryption~\cite{daemen1999aes}, matrix multiplication~\cite{Karpathy}), ISP outperforms OSP by 20\% by avoiding host-SSD transfers, but ISP's limited SIMD parallelism constrains the throughput. 
IFP outperforms both OSP and ISP (50\% improvement over OSP) by exploiting the massive bit- and array-level parallelism of flash arrays. 
Combining IFP and ISP provides additional performance gains because: (i) ISP handles control-intensive operations and complex operations that IFP does not support, and (ii) IFP accelerates bulk data-parallel computation. This result demonstrates that leveraging multiple computation resources mitigates the limitations of individual computation paradigms.

\head{Mixed Workloads} 
For workloads (e.g., aggregation~\cite{soysal2025mars}, sorting~\cite{soysal2025mars}) that involve both computation and data movement, OSP is bottlenecked by host-SSD data transfers.  ISP outperforms OSP by 20\% by reducing the host-SSD communication, but ISP is constrained by the limited SIMD parallelism in the SSD controller cores. 
Combining IFP and ISP improves performance by 40\% over ISP, as IFP accelerates bulk data-parallel computations and ISP efficiently executes control-intensive operations and complex operations that IFP does not support. 

This case study provides three key insights.
First, no single execution model consistently performs well across different workloads. IFP is effective for I/O-intensive workloads where data movement dominates. Combining ISP and IFP is most effective for \rncamiii{the} more compute-intensive and mixed workloads \rncamiii{we examine}. Our case study demonstrates that relying \emph{only} on a single computation resource leads to suboptimal performance across diverse workloads.
% For I/O-intensive workloads, eliminating data movement is critical, which makes IFP the most effective option. For more compute-intensive workloads, combining ISP and IFP exploits the massive internal parallelism of SSD and general-purpose computation capability of SSD controller cores. In hybrid workloads, neither data movement nor computation alone dominates, where combining IFP and ISP improves performance. These results demonstrate that SSD computation resources have complementary strengths, and relying on a single computation resource leads to suboptimal performance. 
Second, performance bottlenecks shift across execution models. OSP's performance is limited by host-SSD data movement. ISP's performance is constrained by its limited SIMD parallelism, and IFP by its limited operation set. These bottlenecks are workload-dependent and can vary even within different execution phases of the same workload.  
% reduces data movement but becomes compute-bound due to limited SIMD parallelism. IFP eliminates data movement, but it is constrained by the limited set of operations it supports. These bottlenecks are workload-dependent and changes even within the same application.
Third, combining multiple SSD computation resources provides benefits, but only when done judiciously.
Naively combining ISP and IFP does not always provide performance gains. In I/O-intensive workloads, combining ISP and IFP leads to additional inter-resource data movement.
% In more compute-intensive and hybrid workloads, coordinated use of computation resources overcomes their individual limitations and delivers performance improvements. 
% This case study shows that offloading across multiple SSD computation resources is necessary because relying on a single resource leads to data movement and computation bottlenecks.
% This case study demonstrates that effective SSD-based NDP requires coordination of when, where, and how computations should be offloaded across SSD's computation resources under varying workload characteristics and system conditions.

This case study demonstrates that effective SSD-based NDP requires fine-grained, workload- and system-aware coordination across multiple heterogeneous SSD computation resources.

\begin{figure*}[b]
\centering
\includegraphics[width=\textwidth]{images/motivation_offloading.pdf}
\caption{Speedup of GPU, \isp{}, \pud{}, \fc{}, \af{}, \bw{}, \dm{} normalized to \cpu{}.}
\label{fig:motivation_prior_offloading}
\end{figure*}

\subsection{Effectiveness of Prior Offloading Approaches \label{subsec:motivation_effectiveness}}
\head{NDP Offloading Techniques} To our knowledge, \emph{no} prior work explores general-purpose, application-transparent offloading of computations across multiple heterogeneous SSD computation resources. 
Several prior techniques (e.g.,~\cite{hsieh.isca16, yang2023lambda, ghiasi2022alp, wolski2008using, hadidi2017cairo, wu2020tuning, alsop2024pim, kim2017toward, wei2022pimprof,jiang20243}) explore partitioning and mapping application code segments for execution between host and NDP units near main memory (e.g., 3D stacked memory with general-purpose cores in its logic layer). These techniques make offloading decisions using a narrow set of system-level characteristics, and do not account for the heterogeneity of SSD computation resources.   
We categorize these techniques into two classes: (1) \textbf{\bw{}}: techniques (e.g.,~\cite{hsieh.isca16, yang2023lambda, wolski2008using,  hadidi2017cairo, wu2020tuning, alsop2024pim}) that make offloading decisions based on bandwidth utilization of the host and NDP units, and (2) \textbf{\dm{}}: techniques (e.g.,~\cite{ghiasi2022alp, kim2017toward, wei2022pimprof,jiang20243}) that prioritize minimizing data movement cost when executing application code across host and NDP units. 

\head{Methodology}
To evaluate the effectiveness of these prior offloading models when adapted to SSD-based NDP, we extend both \bw{} and \dm{} models to utilize all three SSD computation resources.
We implement these approaches in our in-house event-driven simulator and evaluate them across six real-world workloads (see \S\ref{sec:methodology} for our evaluation methodology and workload characteristics).
We compare their performance against:
(1) host CPU and GPU, 
(2) standalone NDP techniques (see \S\ref{subsec:background_ndp}) - \isp{}, \pud{}, \fc{}, and \af{}, and 
(3) an \ideal{} approach that assumes (i) no resource contention (for both computation resources and shared channels), (ii) zero data movement latency to move the operands to the target computation resource, and (iii) the selection of a computation resource that provides the lowest computation latency.

\head{Performance Analysis} \fig~\ref{fig:motivation_prior_offloading} shows the speedup of GPU, \isp{}, \pud{}, \fc{}, \af{}, \bw{}, \dm{} and \ideal{} normalized to \cpu{}.

We make four key observations.
First, \dm{} is the best-performing prior NDP offloading technique with an average speedup of 2.3$\times$ over CPU, 1.0$\times$ over GPU, 1.8$\times$ over \isp{}, 1.3$\times$ over \pud{}, 1.9$\times$ over \fc{}, 1.3$\times$ over \af{}, and 1.1$\times$ over \bw{}. 
\dm{}'s benefits come from offloading computation to multiple SSD computation resources based on data movement cost reduction. 
Second, \dm{} falls short of an \ideal{} policy's performance by 2.5$\times$ on average. This is because \dm{} relies on a narrow offloading model that frequently favors \ifp{} to reduce data movement costs. However, repeated offloading to flash chips (i.e., IFP) introduces queueing delays and resource contention, which reduces IFP's effectiveness. 
Third, \bw{} achieves an average speedup of 2.1$\times$ over CPU but underperforms \dm{} by 11\%. \bw{} prefers lightly loaded computation resources based on bandwidth utilization without considering the cost of moving operands across the computation resources. This shows that bandwidth awareness alone is insufficient for SSD-based NDP, where internal data movement and contention can dominate performance.
Fourth, GPU has comparable performance to \dm{}, and even outperforms \dm{} in highly data-parallel workloads (e.g., heat-3D and jacobi-1D). These workloads benefit from GPU's massive SIMD parallelism and wide vector processing units. 

We conclude that prior offloading techniques consider limited factors, which leads to sub-optimal performance compared to an \ideal{} offloading policy. An effective offloading policy must jointly consider computation capability, data locality, and resource contention across heterogeneous SSD computation resources.

%\subsection{Our Goal}
%Based on our analyses in \S\ref{subsec:motivation_casestudy} and  \S\ref{subsec:motivation_effectiveness}, we conclude that prior offloading techniques do not effectively utilize the SSD computation capabilities as they only take into account limited application and system-level factors.

\textbf{Our goal} is to enable programmer-transparent near-data processing in SSDs that (1) schedules and coordinates computation across multiple heterogeneous SSD computation resources, (2) makes offloading decisions that are aware of both workload characteristics and dynamic system conditions, and (3) improves the performance and energy efficiency of a wide range of applications.

% \textbf{Our goal} is to fundamentally mitigate the data movement bottleneck by fully exploiting the combined computational capabilities of an SSD for NDP in a programmer-transparent manner.

\begin{figure}[h]
    \centering
    \includegraphics[width=\linewidth]{images/stop.png}
\end{figure}

==> macros.tex <==
\makeatletter
\g@addto@macro{\normalsize}{%
 \setlength{\abovedisplayskip}{2pt plus 1pt minus 1pt}
 \setlength{\belowdisplayskip}{2pt plus 1pt minus 1pt}
  \setlength{\abovedisplayshortskip}{0pt}
  \setlength{\belowdisplayshortskip}{0pt}
  \setlength{\intextsep}{2pt plus 1pt minus 1pt}
  \setlength{\textfloatsep}{2pt plus 1pt minus 1pt}
  \setlength{\skip\footins}{5pt plus 1pt minus 1pt}}
   \setlength{\abovecaptionskip}{3pt plus 1pt minus 1pt}
   
\setlength{\abovecaptionskip}{0pt plus 1pt minus 1pt}
\setlength{\belowcaptionskip}{0pt plus 1pt minus 1pt}
 % \setlength{\headsep}{2pt}
 \titlespacing\section{20pt}{20pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
 \titlespacing\subsection{0pt}{2pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
 % \titlespacing\subsubsection{0pt}{6pt plus 2pt minus 2pt}{2pt plus 2pt minus 2pt}
% \makeatother
\makeatother

==> sections/00-rev.tex <==
% \hypersetup{
% % colorlinks=true,
% citecolor=blue,
% linkcolor=blue,
% urlcolor=blue
% }
% %\addtolength{\topmargin}{-3in}
% %\addtolength{\textheight}{0.5in}
% % \hypersetup{
% %   colorlinks   = true, %Colours links instead of ugly boxes
% %   urlcolor     = blue, %Colour for external hyperlinks
% %   linkcolor    = blue, %Colour of internal links
% %   citecolor   = blue %Colour of citations
% % }

% %\setstretch{0.833}

% \definecolor{lightblue}{rgb}{0.68, 0.85, 0.9}
% \DeclareRobustCommand{\markq}[1]{{\noindent\textbf{{\sethlcolor{cornflowerblue!40}{\hl{#1}}}}}}
% \DeclareRobustCommand{\markqg}[1]{{\noindent\textbf{{\sethlcolor{cornflowerblue!40}{\hl{#1}}}}}}
% \DeclareRobustCommand{\markqw}[1]{{\noindent\textbf{{\sethlcolor{cyan!40}{\hl{#1}}}}}}
% \newgeometry{top=0.6in, bottom=0.6in, left=0.75in, right=0.75in}
% \twocolumn
% % \definecolor{cornflowerblue}{rgb}{0.35, 0.52, 0.84}
% \definecolor{cornflowerblue}{rgb}{0.39, 0.58, 0.93}
% \definecolor{brandeisblue}{rgb}{0.0, 0.44, 1.0}

% \newcommand\irev[1]{{\color{cornflowerblue}{#1}}} %isca'24 revision
% \newcommand\ireva[1]{{\color{mahogany}{#1}}} %isca'24 revision
% \newcommand\irevb[1]{{\color{darkspringgreen}{#1}}} %isca'24 revision
% \newcommand\irevc[1]{{\color{darkpink}{#1}}} %isca'24 revision

% \newcommand\revid[1]{\todo[linecolor=cornflowerblue,backgroundcolor=cornflowerblue!50,bordercolor=cornflowerblue]{\textcolor{black}{\textbf{#1}  \begin{center}\hyperref[rev]{$\uparrow$}\end{center} }}}

% \newcommand{\circc}[1]{\tikz[baseline=(char.base)]{
%            \node[shape=circle,draw,inner sep=0pt,fill=cornflowerblue!40, text=black] (char) {#1};}}

%==============================================
%\setstretch{0.95}
%%

\newcommand{\codename}{GenPairX\xspace}
\newcommand{\codealg}{GenPair\xspace}

\begin{spacing}{0.92}
\label{rev}

\noindent We sincerely thank the reviewers for their valuable feedback. We have carefully considered and addressed most of the comments, questions, and concerns in the revised paper draft and cover letter.

GenPairX is the first algorithm-hardware co-design specifically tailored for paired-end read mapping. Our approach directly addresses the growing demand for faster and more efficient genomic analysis. Paired-end sequencing dominates current practice, with approximately 90\% of all sequencing data generated on platforms such as Illumina~\cite{illumina_ngs_company_2025}, which exclusively provide paired-end sequencing instruments~\cite{illumina_sequencing_platforms_2025}. Our work therefore targets the most widely used sequencing mode in the industry, offering a practical and scalable solution for modern genomics pipelines.

%GenPairX represents the first algorithm-hardware co-design specifically tailored for paired-end read mapping. This approach aligns with the increasing demand for more efficient genomic analysis.  Paired-end reads are dominant in the industry, with 90\% of sequencing data worldwide produced by platforms like Illumina~\cite{illumina_ngs_company_2025}, which exclusively offer paired-end sequencing devices~\cite{illumina_sequencing_platforms_2025}. 

\noindent Below we summarize our responses to each reviewer's comments.

%In 2024, Illumina reported core revenue of 4.3B USD~\cite{Illuminaearning}, underscoring the substantial market potential for specialized ASIC solutions aimed at accelerating short-read sequencing.


%%

%%

%%
\markqg{A1: How dataset- or application-dependent are GenPairX’s design and fallback decisions, and when can its performance and hardware applicability be considered generalizable?} 
First, we provide a sensitivity analysis on the dataset error rate in \hyperref[A1.1]{A1.1} to evaluate the applicability of \codename{} across current and future datasets with varying error rates. Second, in \hyperref[A1.2]{A1.2}, we detail how \codealg{} can be adapted for long-read mapping.\\ Regardless of read length, modern sequencing platforms continue to push error rates downward, with recent reports demonstrating per-base error rates approaching 0.0005\% for high-accuracy modes~\cite{Cheng2024, Sun2024}. GenPairX is well aligned with this trend: its performance remains stable for per-base error rates below 0.2\%, making it suitable for current and next-generation sequencing technologies with increasingly low error profiles.
%, and in \hyperref[A1.3]{A1.3}, we evaluate the performance of \codename{} on long reads.

%%
\markqg{A2: How does varying the maximum SeedMap size affect accuracy and efficiency, and does 500 remain an optimal choice?} Please refer to \hyperref[A2]{A2} for the new detailed analysis.

%%
\markqg{B1: What is the one-time construction overhead of the SeedMap in terms of latency and memory, how often is it reused, and can this overhead be considered negligible in practice?} 
The human reference genome is updated with a very low frequency---major releases such as GRCh37, GRCh38, and T2T-CHM13 are years apart---so the SeedMap construction cost is paid only once per reference version. In our implementation, the one-time SeedMap build takes approximately 10 minutes and only needs to be regenerated when switching to a different reference. Since the same SeedMap is then reused for thousands of analyses, its amortized latency and memory overhead become negligible in practical genomic workflows.
%The human reference genome is updated very infrequently---major versions like GRCh37, GRCh38, and T2T-CHM13 appear years apart---so the SeedMap, which takes around 10 minutes to build, only needs to be constructed once per version and can be reused over thousands of analyses, making the overhead negligible.
%%

\markqg{B2: Why was a FIFO depth of 500 chosen for the SeedMap, and how do changes in FIFO depth impact read fallback rate, latency, and overall performance?}
 Please refer to \hyperref[B2]{B2} for the new detailed explanation of the SeedMap and to  \hyperref[A2]{A2} for the new sensitivity analysis of the filtering threshold.\\ A FIFO depth of 500 was used to match the filtering threshold of the index. The locations of each seed must be stored until all locations of all seeds from a given pair are extracted, before being processed by the paired-adjacency filtering module.

% Please refer to \hyperref[B2]{B2} for a detailed explanation of our design and to  \hyperref[A2]{A2} for a sensitivity analysis of the filtering threshold.\\ A FIFO depth of 500 was used to match the filtering threshold of the index. The locations of each seed must be stored until all locations of all seeds from a given pair are extracted, before being processed by the paired-adjacency filtering module.We computed that in $5 \times 10^{-7}$\% of cases, the seeds in the index have 500 locations.

%%
\markqg{B3: Can the authors provide stage-wise latency results for key components like SeedMap Query and Light Alignment, in addition to area and power metrics?
} Please refer to \hyperref[B3]{B3} where we added detailed latency result of each \codename{} component.


\markqg{B4: Can the authors compare the performance gains of the algorithms alone versus when combined with the hardware to show the benefits and justify the hardware overhead?}
Please refer to \cref{fig:throughput_e2e} and its discussions where we added the performance results of GenPair running on CPU (i.e., without hardware acceleration).
%%

\markqg{C1: How does NSML compare to CPU-base implementation if NSML also uses DDR5 memory?}  
Please refer to \hyperref[C1]{C1}, where we added an evaluation of \codename{} under different memory technologies. The benefits of NSML are limited when a lower aggregate memory bandwidth is available; however, compared to prior work, its key advantage is the ability to effectively exploit abundant memory bandwidth whenever the underlying memory subsystem provides it.
%When equipped with four channels of DDR5, our design achieves a throughput of 16.91 MPair/s. In comparison, the CPU implementation of NSML, operating with six channels of DDR4, attains a throughput approximately 2.48× higher than the hardware implementation.\\

%Our design achieves a throughput of 16.91 MPair/s when using four channels of DDR5. The CPU implementation of NMSL, running with six channels of DDR4, attains a throughput approximately $2.48\times$ higher than the hardware implementation. \\

%The benefits of NMSL are limited when the number of memory channels is low but compared to the prior work, the main advantage of NMSL is it can effectively use abundant memory bandwidth whenever the underlying memory subsystem allows.
%%

\markqg{C2: Why must a host provide 14.5GB/s bandwidth with 2-bit encoding to saturate GenPairx bandwidth?} 
With 2-bit encoding, each pair of 300 bp reads (150 bp per read) requires 75 bytes. To saturate the bandwidth of \codename{} (192.7 MPair/s), an input data rate of 14.5 GB/s is required.

%%
\markqg{C3: In V.C what is the host in this configuration instance?}
For a PCIe accelerator card, the host can be any CPU that supports PCIe Gen 4 or higher.

%%
\markqg{D1: Long read integration?}

We added \hyperref[D1.1]{D1.1}, where we show how long reads can be chunked into pairs of short reads, allowing us to apply the \textit{Partitioned Seeding}, \textit{SeedMap Query}, and \textit{Paired-Adjacency Filtering} steps of \codealg{}. We evaluate \codename{} on long reads in \hyperref[D1.2]{D1.2}, \hyperref[A1.3]{A1.3}, and \hyperref[D1.3]{D1.3}. Additionally, we provide a more detailed analysis of the impact of error rate on our design.


%%
\markqg{E1: Can the authors clarify their scaling methodology for the FIFO area, as the reported numbers seem underestimated given typical 7nm SRAM cell and peripheral overheads?}

For a fair comparison, we recomputed the scaled values by rounding the technology down to the lower value listed in the table, which yields an upper bound (rather than a lower bound as before). We provided more details on our scaling methods in \hyperref[E1]{E1}. 

%%
\markqg{E2: Have the authors considered the area and power impact of off-chip signal and power pads, as excluding them may overstate the reported advantages?} 
For a fair comparison with the existing hardware accelerators (GenDP and GenCache), we excluded the impact of off-chip signal and power pads, as their reported results also do not account for these effects.

%%
\markqg{E3: Does the reported 63 mm² for GenDP include the area and power of the required HBM module, or are these excluded from the calculations?}
The reported value excludes the area and power of the HBM module. We have revised the manuscript to clarify that the memory subsystem is not part of our hardware contribution. Consistent with prior work, we report the area and power of the proposed accelerator alone; previous designs also excluded external memory technology from their chip-level totals. Furthermore, our approach does not fundamentally rely on HBM. As shown in \hyperref[C1]{C1}, we provide an evaluation of GenPairX using multiple memory technologies to demonstrate that the architecture can operate under different memory configurations.

%The area and power of the HBM module are excluded from our calculations. Our design does not necessarily rely on HBM; in \hyperref[C1]{C1}, we provide an evaluation of GenPairX across different memory technologies.

%\noindent\irev{We improved the writing and will further polish for the final version} 
\end{spacing}

%\setstretch{0.97}


%\setstretch{\baselinestretch}




%\restoregeometry


%\setstretch{0.94}
% \hypersetup{showlinks}
\hypersetup{
% colorlinks=false,
citecolor=blue,
linkcolor=blue,
urlcolor=blue
}
%\addtolength{\topmargin}{3in}
%\addtolength{\textheight}{-0.5in}
\pagebreak


==> tables/evaluation_methodology.tex <==
\begin{table}[ht]
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.2}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{|c|l|}
  \hline
    
  \multirow{5}{*}{
  \centering 
  \shortstack{\textbf{Host CPU} \\ \textbf{(Real System)}}}
  & Intel(R) Xeon(R) Gold 5118 \\ \cline{2-2} 
  & x86-64~\cite{guide2016intel}, 6~cores, out-of-order, 3.2 GHz  \\ \cline{2-2}
  & \emph{L1 Data + Inst. Private Cache:} 32kB, 8-way, 64B line \\ \cline{2-2}
  & \emph{L2 Private Cache:} 256kB, 4-way, 64B line \\ \cline{2-2}
  & \emph{L3 Shared Cache:} 8MB, 16-way, 64B line \\ 
  
  \hline

  \multirow{4}{*}{
  \centering 
  \shortstack{\textbf{Host GPU} \\ \textbf{(Real System)}}}
  & NVIDIA A100 GPU~\cite{a100, choquette2020nvidia}, \\
  & NVIDIA Ampere Architecture~\cite{ampere} (7nm) \\ \cline{2-2} 
  & 108 Streaming Multiprocessors, 1.4 GHz base clock;  \\ \cline{2-2}
  & \emph{L2 Cache:} 40 MB; Main Memory: 40GB HBM2~\cite{lee2016simultaneous, lee201425} \\ 
  
  \hline
  
  \multirow{4}{*}{\centering \shortstack{\textbf{Host Main Memory} \\ \textbf{(Real System)}}}
  & 32GB DDR4-2400, 4~channels, 1 rank, 16 banks; \\ \cline{2-2} 
  & Peak throughput: 19.2 GB/s;  \\ \cline{2-2} 
  & \textbf{Latency:} \texttt{T\textsubscript{bbop}}: 49 ns;  \textbf{Energy:} \texttt{E\textsubscript{bbop}}: 0.864 nJ; \\ 
  & where $bbop$ is bulk bitwise operation \\ \cline{2-2} 
  
  \hline
  
  \multirow{11}{*}{
  \shortstack{\textbf{SSD~\cite{samsung-980pro}} \\ \\ \textbf{(Simulated)}}}
  & 48-WL-layer 3D TLC NAND flash-based SSD; 2 TB\\ \cline{2-2}
  & \textbf{External Bandwidth}: PCIe 4.0, 8GB/s\\ \cline{2-2} 
  & \textbf{NAND Config}: 8 channels; 8 dies/channel; 2 planes/die;\\
  & 2,048 blocks/plane; 196 (4$\times$48) WLs/block; 4 KiB/page\\ \cline{2-2} 
  & \textbf{Flash Channel Bandwidth}: 1.2 GB/s\\ \cline{2-2} 
  & \textbf{Latency}: 
  T\textsubscript{read} (SLC mode): 22.5 $\mu$s~\cite{park2022flash}; \\
  & T\textsubscript{prog} (SLC mode): 400  $\mu$s~\cite{park2022flash}; T\textsubscript{bers} : 3500 $\mu$s~\cite{park2022flash}\\
  & T\textsubscript{AND/OR}: 20 ns~\cite{gao2021parabit}; T\textsubscript{latchtransfer}: 20 ns~\cite{gao2021parabit}; \\  
  &  T\textsubscript{XOR}: 30 ns~\cite{park2022flash}; T\textsubscript{DMA}: 3.3 $\mu$s;\\\cline{2-2} 
  & \textbf{Energy}: \texttt{E\textsubscript{read}} (SLC mode): 20.5$\mu$J/channel ~\cite{park2022flash}; \\ &
  E\textsubscript{AND/OR}: 10nJ/KB~\cite{gao2021parabit}; E\textsubscript{latchtransfer}: 10nJ/KB~\cite{gao2021parabit}; 
  \\ & E\textsubscript{XOR}: 20nJ/KB~\cite{park2022flash}; E\textsubscript{DMA}: 7.656$\mu$J/channel; \\

  \hline

  \multirow{4}{*}{\centering \shortstack{\textbf{SSD DRAM} \\ \textbf{(Simulated)}}} 
  & 2GB LPDDR4-1866 DRAM cache;\\
  & 1 channel, 1 rank, 8 banks\\ \cline{2-2} 
  & \textbf{Latency:} T\textsubscript{bbop}: 49 ns;  \textbf{Energy:} E\textsubscript{bbop}: 0.864 nJ; \\ 
  & where $bbop$ is bulk bitwise operation \\ 
  \hline 
  
  \textbf{SSD Controller Cores}
  & ARM Cortex-R8 series @1.5GHz; 5 Cores~\cite{arm-cortexR8} \\
  
  \hline
  
  \end{tabular}
  }
\vspace{0.5em}
\caption{Evaluated Configurations.}
\label{tab:eval_config}
\end{table}

==> tables/evaluation_utilization.tex <==
\begin{table}[h]
\centering
\caption{Latency and Core Utilization for ADD32 and MUL32 Operations}
\begin{tabular}{l|ccc|ccc}
\toprule
\multirow{2}{*}{\textbf{Technique}} & \multicolumn{3}{c|}{\textbf{ADD32}} & \multicolumn{3}{c}{\textbf{MUL32}} \\
 & Flash Chips & SSD DRAM & Controller Cores & Flash Chips & SSD DRAM & Controller Cores \\
\midrule
ISP & 0.173030232 & 0.000612374 & 82.6\% & 0.173030232 & 0.000612374 & 82.6\% \\
PuD-SSD & 0.999027994 & 0.000972006 & 0.0\% & 0.999027994 & 0.000972006 & 0.0\% \\
Flash-Cosmos & 0.173030232 & 0.000612374 & 82.6\% & 0.173030232 & 0.000612374 & 82.6\% \\
Ares-Flash & 1 & 0 & 0.0\% & 1 & 0 & 0.0\% \\
\bottomrule
\end{tabular}
\end{table}

==> tables/methodology_baselines.tex <==
\begin{table}[ht]
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.3}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{c|l}
  \hline
  \multirow{5}{*}{\centering \shortstack{\textbf{Host CPU}}}
  & Intel(R) Xeon(R) Gold 5118 \\ \cline{2-2} 
  & x86-64~\cite{guide2016intel}, 6~cores, out-of-order, 3.2 GHz  \\ \cline{2-2}
  & \emph{L1 Data + Inst. Private Cache:} 32kB, 8-way, 64B line \\ \cline{2-2}
  & \emph{L2 Private Cache:} 256kB, 4-way, 64B line \\ \cline{2-2}
  & \emph{L3 Shared Cache:} 8MB, 16-way, 64B line \\ 
  \hline
  \multirow{4}{*}{\centering \shortstack{\textbf{Host Main Memory}}}
  & 32GB DDR4-2400, 4~channels, 1 rank, 16 banks; \\ \cline{2-2} 
  & Peak throughput: 19.2 GB/s;  \\ \cline{2-2} 
  & \textbf{Latency:} \texttt{T\textsubscript{bbop}}: 49 ns;  \textbf{Energy:} \texttt{E\textsubscript{bbop}}: 0.864 nJ; \\ 
  & where $bbop$ is bulk bitwise operation \\ \cline{2-2} 
  \hline
  \multirow{2}{*}{\centering \shortstack{\textbf{Storage (SSD)}}} & Samsung 980 Pro PCIe 4.0 NVMe SSD 2 TB~\cite{samsung-980pro} \\ \cline{2-2} 
  & External PCIe Bandwidth: 8GB/s \\ \cline{2-2}
  \hline
  \end{tabular}
  }
\vspace{0.5em}
\caption{Baseline system configuration.}
\label{tab:config1}
\end{table}

==> tables/methodology_ssd.tex <==
\begin{table}[ht]
  % \vspace{-2mm}
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1.3}
  \resizebox{\columnwidth}{!}{
  \begin{tabular}{|c|l|}
  \hline
  \multirow{9}{*}{
  \centering 
  
  \shortstack{\textbf{SSD NAND} \\ \textbf{Flash Configuration}}}
  & 48-WL-layer 3D TLC NAND flash-based SSD; 2 TB\\ \cline{2-2} 
  & \textbf{NAND Config}: 8 channels; 8 dies/channel; 2 planes/die;\\
  & 2,048 blocks/plane; 196 (4$\times$48) WLs/block; 4 KiB/page\\ \cline{2-2} 
  & \textbf{NAND-Flash Channel Bandwidth}: 1.2-GB/s\\ \cline{2-2} 
  & \textbf{Latency}: \texttt{T\textsubscript{read}} (SLC mode): 22.5 $\mu$s~\cite{park2022flash}; \texttt{T\textsubscript{AND/OR}}: 20 ns~\cite{gao2021parabit}; \\  
  & \texttt{T\textsubscript{latchtransfer}}: 20 ns~\cite{gao2021parabit}; \texttt{T\textsubscript{XOR}}: 30 ns~\cite{park2022flash}; \texttt{T\textsubscript{DMA}}: 3.3 $\mu$s;\\\cline{2-2} 
  & \textbf{Energy}: \texttt{E\textsubscript{read}} (SLC mode): 20.5$\mu$J/channel ~\cite{park2022flash}; \\ &
  \texttt{E\textsubscript{AND/OR}}: 10nJ/KB~\cite{gao2021parabit}; \texttt{E\textsubscript{latchtransfer}}: 10nJ/KB~\cite{gao2021parabit}; 
  \\ & \texttt{E\textsubscript{XOR}}: 20nJ/KB~\cite{park2022flash}; \texttt{E\textsubscript{DMA}}: 7.656$\mu$J/channel; \\ 
  
  \hline
  \multirow{4}{*}{\centering \shortstack{\textbf{SSD Internal DRAM}}} 
  & 2GB LPDDR4-1866 DRAM cache;\\
  & 1 channel, 1 rank, 8 banks\\ \cline{2-2} 
  & \textbf{Latency:} \texttt{T\textsubscript{bbop}}: 49 ns;  \textbf{Energy:} \texttt{E\textsubscript{bbop}}: 0.864 nJ; \\ 
  & where $bbop$ is bulk bitwise operation \\ 
  \hline 
  \textbf{Controller Cores}
  & ARM Cortex-R5 series @1.5GHz; 5 Cores~\cite{arm-cortexR5} \\
  \hline
  
 \end{tabular}
 }
\vspace{0.5em}
\caption{Simulated SSD configuration.}
\label{tab:config2}
\end{table}

==> tables/motivation_utilization.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{2pt}
  \resizebox{\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{NDP Technique} & 
\begin{tabular}{c}    
\textbf{Flash Chips}
\end{tabular} & 
\begin{tabular}{c}    
\textbf{SSD DRAM}
\end{tabular} &
\makecell[c]{
\begin{tabular}{c} 
\textbf{Embedded Cores}
\end{tabular}} \\

\hline
\hline

\textbf{\isp{}} &  
0.25\% & 
0.1\% &
\begin{tabular}{c}
99.74\%
\end{tabular} \\

\hline

\textbf{\pud{}} & 
67.17\%  &
\begin{tabular}{c}
32.83\%
\end{tabular} & 
\begin{tabular}{c}
0\%
\end{tabular} \\

\hline

\textbf{\fc{}} & 
0.25\%  &
\begin{tabular}{c}
0.1\%
\end{tabular} &
\begin{tabular}{c}
99.74\%
\end{tabular} \\

\hline

\textbf{\af{}} & 
99.98\%  &
\begin{tabular}{c}
0.02\%
\end{tabular} &
\begin{tabular}{c}
0\%
\end{tabular} \\

\hline

\end{tabular}
}
\vspace{0.25em}
\caption{SSD compute unit utilization during addition.}
\label{tab:motivation_utilization}
\end{table}


==> tables/offloader_metadata.tex <==
\begin{table}[h]
\centering
\setlength{\tabcolsep}{2pt}
  \resizebox{\linewidth}{!}{%
\begin{tabular}{|c|l|}
\hline
\textbf{Feature} &
\makecell[c]{\textbf{Description}} \\
\hline
\textbf{Operation Type} & 
\begin{tabular}{l}
Type of operation \\(e.g., addition, multiplication)
\end{tabular}
\\
\hline
\textbf{Operand Location} & 
\begin{tabular}{l}
Current location of the operand \\(i.e., flash chips or DRAM)
\end{tabular}
\\
\hline
\textbf{Data Dependency Delay ($delay_{dd}$)}&
\begin{tabular}{l}
Delay for operand availability \\ and the dependent operations 
\end{tabular}
\\
\hline
\begin{tabular}{l}
\textbf{Resource Utilization ($delay_{queue}$)}
\end{tabular}
&
\begin{tabular}{l}
Number of pending requests \\ in each compute unit
\end{tabular}
\\
\hline
\begin{tabular}{c}
\textbf{Data Movement Latency} \\ ($latency_{dm}$)
\end{tabular}
&
\begin{tabular}{l}
Data movement latencies if the operands \\ are not in the target compute unit
\end{tabular}
\\
\hline
\begin{tabular}{c}
\textbf{Expected Computation Latency} \\ ($latency_{comp}$)
\end{tabular}
&
\begin{tabular}{l}
The minimum computation latency \\ based on each compute unit.
\end{tabular}
\\ 
\hline
\end{tabular}
}
\vspace{0.5em}
\caption{Features Used by the Cost Function to Select the SSD Computation Resource.}
\label{tab:offloader_parameters}
\end{table}


==> tables/workloads.tex <==
\begin{table}[h]
    \centering
    \setlength{\tabcolsep}{2pt}
    \scriptsize
    \resizebox{\linewidth}{!}{
    	\begin{tabular}{|c||c|c|c|c|c|}\hline
    	\begin{tabular}{c}\textbf{Workload} \end{tabular} &	
        \begin{tabular}{c}\textbf{Vectorizable} \\ \textbf{Code\%} \end{tabular} 
        & \textbf{Avg. Reuse} & 
            \begin{tabular}{c}    
            \textbf{Low} \\\textbf{Latency} \\\textbf{Operations}
            \end{tabular} &
            \begin{tabular}{c}    
            \textbf{Medium} \\\textbf{Latency} \\\textbf{Operations}
            \end{tabular}
             &
             \begin{tabular}{c}    
            \textbf{High} \\\textbf{Latency} \\\textbf{Operations}
            \end{tabular}
            &
            \hline
                            
            \begin{tabular}{c}\textbf{AES}
            \end{tabular}
            & 65\% & 15.2 & 87\% & 13\% & 0\% \\\cline{2-6}\hline

            \begin{tabular}{c}\textbf{XOR-Filter}
            \end{tabular}
            & 16\% & 2.0 & 1\% & 98\% & 1\% \\\cline{2-6}\hline

            \begin{tabular}{c}\textbf{heat-3D}
            \end{tabular}
            & 95\% & 16 & 0\% & 60\% & 40\% \\\cline{2-6}\hline

            \begin{tabular}{c}\textbf{jacobi-1D}
            \end{tabular}
            & 95\% & 3 & 0\% & 67\% & 33\% \\\cline{2-6}\hline

            \begin{tabular}{c}\textbf{LlaMA2} \\ \textbf{Inference}
            \end{tabular}
            & 70\% & 1.8 & 0\% & 53\% & 47\% \\\cline{2-6}\hline

            \begin{tabular}{c}\textbf{LLM} \\ \textbf{Training}
            \end{tabular}
            & 60\% & 5.2 & 0\% & 88\% & 12\% \\\cline{2-6}\hline
                
    	\end{tabular} 
	}
    \vspace{0.5em}
    \caption{Characteristics of the evaluated workloads.} 
    \label{tab:workloads_characterization}
\end{table}


==> tables/workloads_v0.tex <==
\begin{table}[h]
  \centering
  \footnotesize
  \renewcommand{\arraystretch}{1}
  \begin{tabularx}{\linewidth}{|>{\centering\arraybackslash}m{1.0cm}||>{\centering\arraybackslash}m{1.0cm}|>{\centering\arraybackslash}m{1.0cm}|>{\centering\arraybackslash}m{1.0cm}|>{\centering\arraybackslash}m{1.0cm}|>{\centering\arraybackslash}m{1.2cm}|}
    \hline
    \textbf{Workload} & \textbf{Avg. Reuse} & \textbf{Low Lat. Ops (Bool., read, shift)} & \textbf{Medium Lat. Ops (add., sub., pred.)} & \textbf{High Lat. Ops (mul., div.)} & \textbf{Single /Multiple Units} \\
    \hline\hline
    AES & 15.2 & 87\% & 13\% & 0\% & Single \\
    \hline
    XOR-FILTER & 2.0 & 1\% & 98\% & 1\% & Single \\
    \hline
    heat-3d & 16 & 0\% & 60\% & 40\% & Multiple \\
    \hline
    jacobi-1d & 3 & 0\% & 67\% & 33\% & Multiple \\
    \hline
    LlaMA2 Inference & 1.8 & 0\% & 53\% & 47\% & Multiple \\
    \hline
    LLM Training & 5.2 & 0\% & 88\% & 12\% & Multiple \\
    \hline
  \end{tabularx}
  \vspace{1em}
  \caption{Characterization of workloads.}
  \label{tab:workloads}
\end{table}

